Unsupervised Change Detection in Satellite Images with Generative Adversarial Network

Detecting changed regions in paired satellite images plays a key role in many remote sensing applications. The evolution of recent techniques could provide satellite images with very high spatial resolution (VHR) but made it challenging to apply image coregistration, and many change detection methods are dependent on its accuracy.Two images of the same scene taken at different time or from different angle would introduce unregistered objects and the existence of both unregistered areas and actual changed areas would lower the performance of many change detection algorithms in unsupervised condition.To alleviate the effect of unregistered objects in the paired images, we propose a novel change detection framework utilizing a special neural network architecture -- Generative Adversarial Network (GAN) to generate many better coregistered images. In this paper, we show that GAN model can be trained upon a pair of images through using the proposed expanding strategy to create a training set and optimizing designed objective functions. The optimized GAN model would produce better coregistered images where changes can be easily spotted and then the change map can be presented through a comparison strategy using these generated images explicitly.Compared to other deep learning-based methods, our method is less sensitive to the problem of unregistered images and makes most of the deep learning structure.Experimental results on synthetic images and real data with many different scenes could demonstrate the effectiveness of the proposed approach.

==> sections/backup.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/30/2016_30.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/30/2017_30.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/30/30_refdiff.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/30/gen_30_1.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/30/gen_30_2.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/30/acc_30.png}
    }
    \end{subfigure}
    
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/147/2016_147.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/147/2017_147.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/147/147_refdiff.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/147/gen_147_1.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/147/gen_147_2.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/147/acc_147.png}
    }
    \end{subfigure}
    
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/186/2016_186.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/186/2017_186.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/186/186_refdiff.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/186/gen_186_1.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/186/gen_186_2.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/186/acc_186.png}
    }
    \end{subfigure}
    
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/1243/2016_1243.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/1243/2017_1243.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}{
        \includegraphics[width=1in]{../img_pack/1243/1243_refdiff.jpg}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/1243/gen_1243_1.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/1243/gen_1243_2.png}
    }
    \end{subfigure}
    \hspace{-0.55cm}
    \begin{subfigure}[]{
        \includegraphics[width=1in]{../img_pack/1243/acc_1243.png}
    }
    \end{subfigure}
    \caption{to fit}
    \label{fig:many_exam}
\end{figure*}



Supervised and unsupervised techniques are both commonly used in change detection.
Supervised methods transform change detection task to a classification problem that divides each pixel into two classes, changed or not\cite{camps2008kernel}.
With the development of deep convolutional neural network (CNN), many deep learning structures like U-Net\cite{unet++} and CGAN\cite{cgan} are proposed. 
These methods treated change detection task as ordinary segmentation task in image processing, so they relied heavily on the labels and also required lots of training data, but the former are difficult to obtain.
Thus, despite supervised methods often lead to good results, much attention has been paid to unsupervised ones.

Unsupervised methods are usually based on the concept of Change Vector Analysis (CVA)\cite{cva}, which aims at rating each pixel the possibility of change. These methods can be further divided into two main types, pixel-based and object-based, according to different rating procedures.
Pixel-based methods treat pixels as independent individuals. PCA-Kmeans method\cite{pca-kmeans} applied Principal Component Analysis on the difference map acquired by subtracting corresponding pixels in paired images, then Kmeans-cluster were applied to divide pixels into different classes.
\textsl{C. Wu et al.} \cite{sfa} followed the idea of Slow Feature Analysis (SFA), finding a new space in which most of the pixels are invariant.
\textsl{F. Thonfeld et al.} \cite{rcva} introduced Robust CVA to mitigate the effects of pixel neighbourhood.
Pixel-based methods can have lots of data to analysis but could be affected by noise pixels or might lose much information between pixels.
Object-based change detection methods take spatial context information into account\cite{object-oriented2001} and various algorithms are developed to segment objects of interest\cite{object-based2008} \cite{object-based2012} \cite{object-based2018}. \textsl{L. Li et al.} \cite{ocva} proposed object-oriented CVA  to compare each segment rather than single pixel. However, their results depend on the efficiency of segmentation process, which is still worthy of research.
In addition, some other types of change detection methods are developed, key points matching is one of them.
\textsl{G. Liu et al.} \cite{contrario} proposed to compute mappings between two images using SIFT\cite{sift}-like descriptors extraction and matching, then changed regions were indicated by mismatched descriptors.

Many of these unsupervised methods rely on the image coregistration that guarantees pixels, which have the same coordinates in two paired images, representing the same object.
But co-registered pairs are nearly impossible to obtain in real cases. 
Nowadays, the satellite images describing the same scene may be taken by different sensors, from different angles or at different time in a day. Fig. \ref{fig:uncor_illu} shows an example of unregistered scenes. The different appearances of the same buildings made the corresponding pixels apparently different and could also lead to different segmentation outputs. The corresponding shadows have similar appearances but different coordinates. 
Many of the unregistered objects are dispersed across the whole images and existing coregistration methods could not handle these cases even if more additional information is provided. Thus, it is hard to obtain coregistered pairs and results of change detection methods could be affected heavily.

With CNNs shows strong capacity for extracting high-level features that are semantically rich, deep-learning structures are applied into unsupervised methods to alleviate the effect of unregistered problems. Complex analysis on the abstract representation of the scene acquired via CNNs would be performed to generate change map.
\textsl{J. Liu et al.} \cite{bipartite} proposed an unsupervised method based on Restricted Boltzmann Machine to project the images into a low-dimension vector space, then change map can be generated by making the images' feature vectors much more similar.
\textsl{B. Du et al.} \cite{dsfa} proposed exploiting neural network to implement Slow Feature Analysis process.
\textsl{S. Saha et al.} \cite{unsupervisedCVA} used a pre-trained CNN to outcome feature vector, and a specific comparison and selection process was adopted.
\textsl{N. Lv et al.} \cite{autoencoders} introduced Contractive Autoencoder for extracting features from multiple images metrics. 
